Syntax-augmented Multilingual BERT for Cross-lingual Transfer

In recent years, we have seen a colossal effort in pre-training multilingual text encoders using large-scale corpora in many languages to facilitate cross-lingual transfer learning. However, due to typological differences across languages, the cross-lingual transfer is challenging. Nevertheless, language syntax, e.g., syntactic dependencies, can bridge the typological gap. Previous works have shown that pre-trained multilingual encoders, such as mBERT \cite{devlin-etal-2019-bert}, capture language syntax, helping cross-lingual transfer. This work shows that explicitly providing language syntax and training mBERT using an auxiliary objective to encode the universal dependency tree structure helps cross-lingual transfer. We perform rigorous experiments on four NLP tasks, including text classification, question answering, named entity recognition, and task-oriented semantic parsing. The experiment results show that syntax-augmented mBERT improves cross-lingual transfer on popular benchmarks, such as PAWS-X and MLQA, by 1.4 and 1.6 points on average across all languages. In the \emph{generalized} transfer setting, the performance boosted significantly, with 3.9 and 3.1 points on average in PAWS-X and MLQA.

==> figures/mtop.tex <==
\begin{figure}
\centering
\includegraphics[width=1.0\linewidth]{images/mtop.png}
\caption{MTOP results.}
\label{figure:mtop}
% \vspace{-2mm}
\end{figure}

\begin{figure*}
\centering
\includegraphics[width=0.8\linewidth]{images/wikiann.png}
\caption{
Cross-lingual NER performance (F1) difference (on test set) of mBERT using {\tt Wikiann} dataset \cite{pan-etal-2017-cross} across 20 languages. 
Positive difference indicates that incorporation of syntax improve performance and vice versa.
The dotted vertical lines separate the languages into families: IE.Germanic (en, de, nl), IE.Romance (es, fr, pt), IE.Slavic (bg, ru), IE.Greek (el), IE.Indic (hi, ur), Uralic, (et, fi, hu) Afro-Asiatic (ar, vi), Dravidian (ta, te), Altaic (tr), and Korean (ko). 
}
\label{figure:mtop}
% \vspace{-2mm}
\end{figure*}

